From Continual Learning to Causal Discovery in Robotics

Reconstructing accurate causal models of dynamic systems from time-series of sensor data is a key problem in many real-world scenarios. In this paper, we present an overview based on our experience about practical challenges that the causal analysis encounters when applied to autonomous robots and how Continual Learning~(CL) could help to overcome them. We propose a possible way to leverage the CL paradigm to make causal discovery feasible for robotics applications where the computational resources are limited, while at the same time exploiting the robot as an active agent that helps to increase the quality of the reconstructed causal models.

==> sections/04_approach.tex <==
\section{Causal Robot Discovery} \label{sec:approach}

A review of the literature revealed that the possible limitations of autonomous robots doing causal discovery with their own on-board sensors have not been taken into account. Indeed, the computational and memory requirements for long time-series of sensor data are often very demanding, making the use of previous algorithms for causal inference unfeasible on such platforms.

Our approach is partially inspired by the works of~\citet{8999127} for handling non-stationary data, but differs from it in two ways. First of all, we adopt the current state-of-the-art PCMCI method for causal discovery from time-series data; second, we propose to re-learn the causal model not only when the observed scenario changes, but also at each new robot's set of observations/interventions (periodically, e.g. every few minutes). In particular, the introduction of the CL paradigm could help the robot to overcome the challenge of limited hardware resources and to improve the quality of the causal analysis even with non-stationary data. In addition, a CRD approach could benefit from the fact that robots are physically embodied in the environment and can actively influence its dynamic processes (i.e. by performing interventions). That is, CRD could improve the accuracy of the causal model by enriching ``passive'' observational data from the sensors with ``active'' interventional data from robot's actions aimed at collecting specific time-series for causal discovery.

Therefore, our goal is to decrease the need of hardware resources -- often scarce in autonomous systems -- and to increase the causal analysis quality by using the robot as an active agent in the learning process. The use of CRD would allow the creation of high quality causal models by continually updating them with new sensor data from robot's observations and interventions, without the need to re-process the whole time-series but only new information in an incremental fashion.
The CRD system envisaged in this paper
%The proposed CRD system 
is thought to limit the demand for hardware resources and allow the robot to perform high quality causal discovery in a reasonable time by using its own on-board sensor data.

The proposed approach is depicted in Fig.~\ref{fig:approach}: (\textit{i}) starting from a prefixed set of variables, the robot collects meaningful data by observing and intervening in the target scenario; %Since the autonomous robot can not rely on external resources, the size of the time-series is strictly related to the hardware resources at its disposal and on the possibility to perform a causal analysis in a feasible time;
(\textit{ii}) based on this data, a causal model is estimated using PCMCI~\cite{runge_causal_2018}, which computes test statistics and p-values as causal strengths of the DAG's links.
At this stage, differently from \cite{8999127}, to increase the accuracy of the causal discovery, the robot keeps on collecting data by observing and intervening in the scenario to create new causal models. Periodically then, the robot compares the new causal models with the old ones, inheriting from the latter only the links that minimise the p-values of the DAG's causal relations. By repeating this process until the observed scenario changes, a stable version of the causal model with minimum uncertainty levels would be reached. The latter is useful not only for modeling the current scenario, but also when it changes. Indeed, by partially using the stored causal model that is consistent the target scenario, even the latter changes, the estimation of the new model can be significantly sped up~\cite{8999127}.

Note that by iteratively discarding the old time-series and storing only the built causal model helps to avoid the combinatorial explosion otherwise affecting the PCMCI discovery, therefore allowing the robot to operate and compute new models within reasonable time.
The catastrophic-forgetting problem is also mitigated by the fact that, during continuous operations, the robot observes similar processes with only small incremental changes, which leads to sequences of similar causal models, and that it reconstructs the latter by exploiting relatively small variations of the previous models.

\begin{figure}[t]\centering
\includegraphics[trim={0cm 0cm 5cm 7cm}, clip, width=\columnwidth]{resource/approach.pdf}
\caption{CRD approach: the robot provides observational and interventional data about the human-object interaction to the CRD block. The latter generates a causal model which is stored and used to compare the next causal model built on the next robot's observation and intervention.}
\label{fig:approach}
\end{figure}


